SoK: A Taxonomy for Critical Analysis of Consensus Mechanisms in Consortium Blockchain

Consensus algorithms are central to blockchain technology and an emerging research area. In this paper, we begin with an overview of the different types and architectures of blockchain networks. Then, with a focus on consortium blockchains, we survey, classify, and assess their principal consensus mechanisms. Furthermore, as consensus mechanisms determine network reliability, enhance performance efficiency, and ensure system security, we conduct a critical analysis of the strengths and weaknesses of consensus algorithms using a taxonomy of three different criteria: reliability, performance, and security. We conclude with insights into current and future research challenges and opportunities in this domain.

==> algorithms/hotstuff.tex <==
It uses a parallel pipeline to process a proposal, which is equivalent to combining the preparation and commitment phases of PBFT. The original proposal includes two implementations of HotStuff, Basic HotStuff, and Chained HotStuff. The Basic HotStuff protocol forms the core of HotStuff, which switches between a series of views. The views switch according to a monotonically increasing number sequence. A unique consensus leader exists within each view. Each replica maintains a tree structure of pending commands in its memory. Uncommitted branches compete, and only one branch in a round will be agreed upon by the nodes. In the HotStuff protocol, branches are committed as the view number grows. Voting in HotStuff uses the cryptographic term \textsf{Quorum Certificate} (\textsf{QC}), where each view is associated with a \textsf{QC} that indicates whether enough replicas have approved the view. If a branch is confirmed by a replica, it signs the branch, creates a partial certificate \cite{Chan_Pass_Shi}, and sends to the leader. The leader collects $n - f$ partial certificates, which can be combined into a \textsf{QC}. A view with a \textsf{QC} means that it received the majority votes of the replicas. The leader collects signatures from $n-f$ replicas by using threshold signatures \cite{cachin_blockchain_2017,Gueta_Abraham_Grossman_Malkhi_Pinkas_Reiter_Seredinschi_Tamir_Tomescu_2019}. The algorithm consists of five phases: \textbf{Prepare}, \textbf{Pre-prepare}, \textbf{Commit}, \textbf{Decide} and \textbf{Finally}, as shown in Figure \ref{fig:bftstyle}. 

(1) \textbf{Prepare}. The leader of the current highest view, initiates a proposal for \textsf{highQC}, encapsulates it into a \textsf{Prepare} message with content $\langle \textsf{Prepare}, \textsf{CurProposal}, \textsf{HighQC}\rangle$, and broadcasts it to all replicas. Replicas decide whether to accept the proposal and return a vote with partial signature to the leader if they accept it. 
(2) \textbf{Pre-commit}. When the leader receives votes from $n-f$ replicas for the current proposal, it combines them into \textsf{PrepareQC}, encapsulates into a \textsf{Pre-commit} message, and broadcasts it to all replicas. Replicas vote after receiving the proposal message and returns the vote to the leader. 
(3) \textbf{Commit}. When the leader receives the \textsf{Pre-commit} votes from $n-f$ replicas, it merges them into \textsf{PrecommitQC}, encapsulates into a \textsf{Commit} message, and broadcasts them to all replicas. The replica votes after receiving the proposal message and returns the \textsf{Commit} vote to the leader. To ensure the safety of the proposal, the replica is locked by setting its \textsf{LockedQC} to \textsf{PrecommitQC}. 
(4) \textbf{Decide}. When the leader receives the \textsf{Commit} votes from $n-f$ replicas, it merges them into one \textsf{CommitQC} and then broadcast it to all replicas using a \textsf{Decide} message. After receiving this message, the replica confirms and submits the proposal in the \textsf{CommitQC}, executes the command, and returns it to the client. The replica increases the \textsf{ViewNumber} and starts the next view.
(5) \textbf{Finally}. If the system moves to the next view, each replica sends a message to the next view's leader with the message $\langle\textsf{New-view}, \textsf{PrepareQC}\rangle$.

To optimize and simplify the protocol, a Chained HotStuff was proposed \cite{Hotstuff_paper}. In this protocol, the leader collects replicas' votes in the \textbf{Prepare}  phase and stores them in a state variable called \textsf{GenericQC}. Then, \textsf{GenericQC} is forwarded to the leader of the next view, delegating the \textbf{Pre-commit} phase responsibilities to them. Thus, the next view's leader executes the \textbf{Pre-commit} phase simultaneously with its own \textbf{Prepare} phase. Specifically, the \textbf{Pre-commit} phase of view $v+1$ also acts as the \textbf{Pre-commit} phase of view $v$, and the \textbf{Prepare} phase of view $v+2$ acts as both the \textbf{Pre-commit} phase of view $v+1$ and the \textbf{Commit} phase of view $v$.

==> bios/fadi.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/fadi.png}}]{Dr. Fadi P. Deek} is a Distinguished Professor at New Jersey Institute of Technology (NJIT) where he began his academic career as a student in the early 1980s. He received his B.S. and M.S. in Computer Science, and PhD in Computer and Information Science; all from NJIT. Dr. Deek’s faculty appointments are in two departments: Informatics (in the College of Computing) and Mathematical Sciences (in the College of Science and Liberal Arts). Dr. Deek also serves as a member of the Graduate Faculty at Rutgers University-Newark. He has similarly progressed through administrative ranks at NJIT, culminating with Provost and Senior Executive Vice President for a decade, and Dean of the College of Science and Liberal Arts the prior decade.
\end{IEEEbiography}


==> bios/renita.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/renita.png}}]{Dr. Renita Murimi} received her PhD and MS in Electrical Engineering from New Jersey Institute of Technology, and a Bachelor of Engineering in Electronics and Communications from Manipal Institute of Technology in India. She is an Associate Professor of Cybersecurity at the University of Dallas. Her current research interests are in the areas of cybersecurity, network science, and computational social science.
\end{IEEEbiography}




==> bios/wang.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/wang.jpg}}]{Dr. Guiling (Grace) Wang} is a distinguished professor of computer science and associate dean for research in the Ying Wu College of Computing at the New Jersey Institute of Technology (NJIT), and the founding director of the NJIT Center for AI Research. She also holds a joint appointment at the MT School of Management. She received a B.S. in Software from Nankai University and a Ph.D. in Computer Science and Engineering, with a minor in Statistics, from Pennsylvania State University. She is a Chartered Financial Analyst (CFA), an IEEE Fellow and a Fellow of the Asia-Pacific Artificial Intelligence Association. Her research interests include FinTech, deep learning, blockchain technologies, and intelligent transportation.
\end{IEEEbiography}





==> bios/wei.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bios/wei.jpg}}]{Wei Yao} received the B.S. degree in Computer Science from Huazhong University of Science and Technology, Wuhan, China, M.S. degree in      Electronic Engineering from University of Hartford, and M.S. degree in Computer Science in Central Connecticut State University. Wei is currently a Ph.D. candidate in Computer Science at New Jersey Institute of Technology. His research interests include Internet of Things, cybersecurity, blockchain technologies and applications in various areas. 
\end{IEEEbiography}
